Silent Self-stabilizing BFS Tree Algorithms Revised

In this paper, we revisit two fundamental results of the self-stabilizing literature about silent BFS spanning tree constructions: the Dolev et al algorithm and the Huang and Chen's algorithm. More precisely, we propose in the composite atomicity model three straightforward adaptations inspired from those algorithms. We then present a deep study of these three algorithms. Our results are related to both correctness (convergence and closure, assuming a distributed unfair daemon) and complexity (analysis of the stabilization time in terms of rounds and steps).

==> s2-correction-CJ.tex <==
\subsection{Partial Correctness}

Below we establish the partial correctness of $\algoU$, $\algoB(D)$,
and $\algoHC(D)$ using three main steps: (1) we define a set of {\em
  legitimate} configurations, (2) we show that a BFS spanning tree is
defined in each legitimate configuration, and (3) we show that every
terminal configuration of each algorithm is legitimate.

\begin{definition}\label{def:legi}
A configuration is {\em legitimate} if and only if for every process
$p$, we have $d_p = \|p,\Root\|$ and $d_{p} = d_{par_p}+1$.
\end{definition}

Let $T_\gamma = (V,E_T)$, where $E_{T_\gamma} = \{\{p,q\} \in E, q
\neq \Root \wedge par_q = p$ in $\gamma\}$.

 
\begin{theorem}\label{bfs:5}
 $T_\gamma$ is a breath-first spanning tree in every legitimate
  configuration $\gamma$.
\end{theorem}
\begin{proof}
Let $\gamma$ be any legitimate configuration.  We first demonstrate
that $T_\gamma$ is a spanning tree by showing the following two
claims:
\begin{description}
\item[$T_\gamma$ is acyclic:] Assume, by contradiction, that
  $T_\gamma$ contains a cycle $p_0,\ldots, p_k, p_0$. By
  definition, $\Root$ is not involved into the cycle. Assume,
  without loss of generality, that for all $i>0$, $par_{p_{i}} =
  p_{i-1}$ et $par_{p_0} = p_{k}$ in $\gamma$. From
  Definition~\ref{def:legi}, in $\gamma$ we have $d_{p_i}>d_{p_{i-1}}$
  and, by transitivity, $d_{p_k} > d_{p_0}$. Now, as $par_{p_0} =
  p_{k}$, we have $d_{p_0} > d_{p_k}$ by Definition~\ref{def:legi}, a
  contradiction.

\item[$|E_{T_\gamma}| = n-1$:] Each edge of $V/{\Root}$ has a single parent.
%\item[$|E_{T_\gamma}| = n-1$:] Following a similar reasoning, each
%  edge of $E_{T_\gamma}$ is pointed by the $Par$-variable of a unique
%  non-root process, indeed suppose the contrary: let two neighbors $p$
%  and $q$ such that (1) $par_p = q$ et (2) $par_q = p$. From
%  Definition~\ref{def:legi}, (1) implies that $d_p > d_q$ and (2)
%  implies that $d_q > d_p$, a contradiction.
%Thus, as there are $n-1$ non-root process, we have $|E_{T_\gamma}| = n-1$.
\end{description}
We now show that $T_\gamma$ is breath-first. 
Let $p_0=\Root, \ldots, p$
the unique path from $\Root$ to $p$ in the tree. 
One can easily establish that $d_{p}$ is the length 
of the path from $\Root$ to $p$ in the tree. 
By Definition~\ref{def:legi}, $d_{p}= \|\Root,p\|$. 
Hence, the length of the path 
from $\Root$ to $p$ in $T_\gamma$  is minimal.
%By definition, for all
%$i>0$, $par_{p_{i}} = p_{i-1}$.  By Definition~\ref{def:legi}, we have
%$d_{p_i}=d_{p_{i-1}}+1$ and, by transitivity,
%$d_{p_k}=d_{p_{0}}+k$. Moreover, $d_{p_0} = d_\Root = 0$. So, $d_{p_k}$ is
%the length $k$ of the path from $\Root$ to $p_k$. Now, by
%Definition~\ref{def:legi}, $d_{p_k}$ is also equal to
%$\|\Root,p_k\|$. Hence, the length $k$ of the path from $\Root$ to $p_k$. is
%equal to the distance from $\Root$ to $p_k$ in $G$.
\end{proof}

Let $D\geq \diam$.  Let $\mathcal{TC}_{\algoU}$,
$\mathcal{TC}_{\algoB(D)}$, and $\mathcal{TC}_{\algoHC(D)}$ be the set of
terminal configurations of $\algoU$, $\algoB(D)$, and $\algoHC(D)$,
respectively.



\begin{lemma}
Let $\gamma$ be a terminal configuration of
$\mathcal{TC}_{\algoU}$. Let $X$ be the largest distance value in $\gamma$.
$\gamma$ is a
terminal configuration of $\mathcal{TC}_{\algoB(X)}$. 
\end{lemma}
\begin{proof}
Any node $p$ in $\gamma$ verifies $dOk(p) \wedge parOk(p)$.
So $p$ does not verify the guard of the rule $B_1$ and $B_3$ 
of $\mathcal{TC}_{\algoB(i)}$ for all $i$.
Any node $p$ in $\gamma$ verifies $\mind(p) < X$.
So $p$ does not verify the guard of the rule $B_3$ 
of $\mathcal{TC}_{\algoB(X)}$.
\end{proof}
\begin{lemma}
Let $D \geq \diam$.
Let $\gamma$ be a non-terminal configuration of $\algoHC(D)$. 
$\gamma$ is a non-terminal configuration of $\algoB(D)$.
\end{lemma}
\begin{proof}
There is a node $p$ such that 
$(\neg parOk(p) \wedge d_{par_p} < D) \vee d_{par_p} > \mind(p)$ is
true in $\gamma$.

Assume first that $\neg parOk(p) \wedge d_{par_p} < D$ is true in $\gamma$. Then,
%$d_{par_p} < D$ implies that 
$\mind(p)<D$ is true, thus either $B_1$
or $B_2$ is enabled in $\gamma$ because $\neg parOk(p)$ is true.

Assume then that $d_{par_p} > \mind(p)$. 
%Then, as $d_{par_p} \leq D$ (by definition), 
We have $\mind(p) < D$. So, if $\neg dOk(p)$, then
$B_1$ is enabled in $\gamma$. Otherwise, we have $d_p =
\mind(p)+1$. So, $d_p \neq d_{par_p}+1$; consequently, $B_2$ is enabled
in $\gamma$.
\end {proof}

Hence, every non-terminal configuration of $\algoHC(D)$ is a
non-terminal configuration of $\algoB(D)$. Thus, we have:
$\mathcal{TC}_{\algoB(i)} \subseteq \mathcal{TC}_{\algoHC(i)}$.

To sum up: 
\begin{remark}\label{rem:term}
$\mathcal{TC}_{\algoU} \subseteq \bigcup_{i=\diam}^\infty
  \mathcal{TC}_{\algoB(i)} \subseteq \bigcup_{i=\diam}^\infty
  \mathcal{TC}_{\algoHC(i)}$.
\end{remark} 

From the previous remark, we know that it is sufficient to show that
any configuration of $\bigcup_{i=\diam}^\infty \mathcal{TC}_{\algoHC(i)}$
is legitimate to establish that any configuration of
$\mathcal{TC}_{\algoU}$, $\bigcup_{i=\diam}^\infty \mathcal{TC}_{\algoB(i)}$, 
and $\bigcup_{i=\diam}^\infty  \mathcal{TC}_{\algoHC(i)}$ are legitimate.

\begin{lemma}\label{lem:leq}
Let $d \geq \diam$.
In any configuration of $\mathcal{TC}_{\algoHC(D)}$ 
we have $d_p \leq \|p,\Root\|$ for every
process $p$.
\end{lemma}
\begin{proof}
Let $\gamma$ be any terminal configuration of $\algoHC(D)$.
We now show that $\gamma$ is legitimate. By
definition, $d_{\Root} = 0$ in $\gamma$.

Assume, by the contradiction, that there is a process $p$ such that
$d_p > \|p,\Root\|$ in $\gamma$.  We have $p\neq R$ and $d_p \geq 1$.
Without loss of generality, assume
$p$ is one of the closest processes from $\Root$ such that $d_p >
\|p,\Root\|$ in $\gamma$. By
definition $\|p,\Root\| \leq \diam$, and $p$ has at
least a neighbor, $q$, such that $\|q,\Root\| = \|p,\Root\|-1 <
\diam$.  By hypothesis, $d_q \leq \|q,\Root\| = \|p,\Root\|-1$ in
$\gamma$.  We have $\mind(p) \leq d_q < \diam$ and $d_p > d_q+1$.
If $d_p = d_{par_p} + 1$ then $HC_2$ is enabled in
$\gamma$, otherwise $HC_1$ is enabled.  
So, $\gamma$ is not terminal, a contradiction. 
%Thus, we can 
%conclude that in a terminal configuration of $\bigcup_{i=\diam}^\infty
%\mathcal{TC}_{\algoHC(i)}$ we have $d_p \leq \|p,\Root\|$ for every
%process $p$.
\end{proof}


\begin{corollary}
\label{cor:leq}
Let $\gamma$ be a terminal of $\mathcal{TC}_{\algoHC(D)}$ where $ D \geq \diam$.
Every node $p \neq \Root$ verifies $d_p = d_{par_p}+1$ and $d_{par_p} = \mind(p)$.
\end{corollary}
\begin{proof}
Every node $p\neq \Root$ has a neighbor such that $\|q,\Root\| \leq \diam -1$.
We have $d_q \leq \diam -1 $ according Lemma \ref{lem:leq}.
We conclude that $\mind(p) \leq \diam -1$.
As $\gamma$ is a configuration terminal, we have 
$d_p = d_{par_p}+1$ and $d_{par_p} = \mind(p)$.
\end{proof}

\begin{lemma}\label{lem:eq}
Let $d \geq \diam$.
In any configuration of $\mathcal{TC}_{\algoHC(D)}$ we have 
$d_p = \|p,\Root\|$ for every process
$p$.
\end{lemma}
\begin{proof}
Let $\gamma$ be any terminal configuration of $\algoHC(D)$.  
Assume, by the contradiction, that there is a process
$p\neq \Root$ such that $d_p \neq \|p,\Root\|$ in $\gamma$. 
By Lemma~\ref{lem:leq}, $d_p <
\|p,\Root\| \leq \diam$ in $\gamma$.  

Without loss of generality, assume that $p$ is the process with the
minimum value of $d_p$ satisfying $d_p < \|p,\Root\|$ in $\gamma$.
According to Corollary \ref{cor:leq}, we have 
$d_{par_p} = mind(p) < D$ and   $d_p = d_{par_p}+1$.
So by hypothesis, we have $d_{par_p} = \|par_p, \Root\|$.
We conclude that $d_p = \|par_p,\Root\|+1 \geq \|p,\Root\|$  
in $\gamma$, a contradiction.
\end{proof}


From the two previous lemmas and Remark~\ref{rem:term}, we can deduce
the following theorem:
\begin{theorem}
Let $d \geq \diam$.
Every configuration of $\mathcal{TC}_{\algoU}$, of 
$\mathcal{TC}_{\algoB(D)}$, and of $\mathcal{TC}_{\algoHC(D)}$ is
legitimate.
\end{theorem}

